Asymptotic Expansions and Bondi Positivity in Higher Dimensional Relativity

The positivity of the Bondi mass has been proven in 4 dimensions, but in higher dimensions the issue remains open. The formalism of the present paper has been developed to investigate this and is well suited to the higher dimensional case. At null infinity, we make asymptotic expansions of the metric components in conformal Gaussian null coordinates, and use the vacuum Einstein equations to solve for the expansion coefficients. We find simple coordinate formulae for the Bondi mass, news and flux in terms of the expansion coefficients of the metric components. We also make expansions of the generator of an asymptotic symmetry and obtain expressions for its expansion coefficients in terms of those of the metric components. We make a spinorial asymptotic expansion of a solution to the Dirac equation in the four dimensional case, and use it to give a clean proof that the Bondi mass is positive in four dimensions. The generalisation to higher dimensions has been investigated, but not yet resolved: indeed, the spinor mass appears to be divergent in the higher dimensional case, because of terms which appear to be singular in the limit at infinity. Such apparently singular terms are common in many of our calculations, but can generally be shown to be zero before the limit is taken. However, it is not yet clear this can be done in the case of the spinor mass in higher dimensions, so further investigation is required.

==> Proofs.tex <==


